Spectral Study of the WNL Star FSZ35 in the M33 Galaxy

We study and analyse low-resolution spectra of the unordinary late WN star FSZ35 in M33. We classify the object as a hydrogen-rich WN8 star. Using the radiative transfer code CMFGEN, we determine the physical parameters of this object and compare them to the parameters of other WN8 stars including the LBV star Romano's star during the minimum of brightness. Unlike Romano's star, the object is fairly stable both spectrally and photometrically, that may be attributed to its more advanced evolutionary stage or lower luminosity. FSZ35 is shown to possess a compact nebula producing faint but detectable [OIII]emission. Location of this object at a large distance (about 100 pc) from the nearest association suggests the object may be one more example of a massive runaway star.

==> reply_Hamann.tex <==
Dear Prof. Dr. Hamann!

We have taken into account for all your comments. Following
corrections were made to the text of the article:

I.
We agree with the  comment about the line widths. 
We calculated models with a higher terminal velocities
and concluded that a model with $v_{\infty}=800 km/s$ fits the
observed spectrum better. Additional mechanisms of broadening are not required. 
Hence we excluded the section ``Line broadening''.

II. Some more recent data on the WN8h stars WR116 and WR89 were added
to table 3.

III. We use the value of 20km/s (2.5\% terminal velocity) for the
turbulent velocity. Its variation does not affect the spectra much
unless the turbulence becomes sufficiently super-sonic. 

IV. We considered the influence of filling-factor and confirm that its
effect on line profiles is difficult to measure at our
resolution. Filling factor is simply fixed to $f=0.1$. For the
mass-loss rate, we finally give two values \dot{M}_{cl} (clumped)
and \dot{M}_{uncl} (unclumped) differing by a factor of $\sqrt{f}$.

V. All the minor remarks were considered, language checked and
improved throughout the text. 

Yours sincerely,
                     Olga Maryeva \& Pavel Abolmasov     

